Enough?

We respond to Aronow et al. (2025)'s paper arguing that randomized controlled trials (RCTs) are "enough," while nonparametric identification in observational studies is not. We agree with their position with respect to experimental versus observational research, but question what it would mean to extend this logic to the scientific enterprise more broadly. We first investigate what is meant by "enough," arguing that this is fundamentally a sociological claim about the relationship between statistical work and larger social and institutional processes, rather than something that can be decided from within the logic of statistics. For a more complete conception of "enough," we outline all that would need to be known -- not just knowledge of propensity scores, but knowledge of many other spatial and temporal characteristics of the social world. Even granting the logic of the critique in Aronow et al. (2025), its practical importance is a question of the contexts under study. We argue that we should not be satisfied by appeals to intuition about the complexity of "naturally occurring" propensity score functions. Instead, we call for more empirical metascience to begin to characterize this complexity. We apply this logic to the example of recommender systems developed by Aronow et al. (2025) as a demonstration of the weakness of allowing statisticians' intuitions to serve in place of metascientific data. Rather than implicitly deciding what is "enough" based on statistical applications the social world has determined to be most profitable, we argue that practicing statisticians should explicitly engage with questions like "for what?" and "for whom?" in order to adequately answer the question of "enough?"

==> abstract.tex <==
We respond to Aronow et al. (2025)'s paper arguing that randomized controlled trials (RCTs) are ``enough," while nonparametric identification in observational studies is not. 
We agree with their position with respect to experimental versus observational research, but question what it would mean to extend this logic to the scientific enterprise more broadly.
We first investigate what is meant by ``enough," arguing that this is a fundamentally a sociological claim about the relationship between statistical work and larger social and institutional processes, rather than something that can be decided from within the logic of statistics. For a more complete conception of ``enough," we outline all that would need to be known -- not just knowledge of propensity scores, but knowledge of many other spatial and temporal characteristics of the social world. Even granting the logic of the critique in Aronow et al. (2025), its practical importance is a question of the contexts under study. We argue that we should not be satisfied by appeals to intuition about the complexity of ``naturally occurring" propensity score functions. Instead, we call for more empirical metascience to begin to characterize this complexity. We apply this logic to the example of recommender systems developed by Aronow et al. (2025) as a demonstration of the weakness of allowing statisticians' intuitions to serve in place of metascientific data. 
Rather than implicitly deciding what is ``enough" based on statistical applications the social world has determined to be most profitable, we argue that practicing statisticians should explicitly engage with questions like ``for what?" and ``for whom?" in order to adequately answer the question of ``enough?"


==> includes.tex <==


\newcommand{\drew}[1]{\textcolor{red}{#1 -Drew~}}

